AppBuddy: Learning to Accomplish Tasks in Mobile Apps via Reinforcement Learning

Human beings, even small children, quickly become adept at figuring out how to use applications on their mobile devices. Learning to use a new app is often achieved via trial-and-error, accelerated by transfer of knowledge from past experiences with like apps. The prospect of building a smarter smartphone - one that can learn how to achieve tasks using mobile apps - is tantalizing. In this paper we explore the use of Reinforcement Learning (RL) with the goal of advancing this aspiration. We introduce an RL-based framework for learning to accomplish tasks in mobile apps. RL agents are provided with states derived from the underlying representation of on-screen elements, and rewards that are based on progress made in the task. Agents can interact with screen elements by tapping or typing. Our experimental results, over a number of mobile apps, show that RL agents can learn to accomplish multi-step tasks, as well as achieve modest generalization across different apps. More generally, we develop a platform which addresses several engineering challenges to enable an effective RL training environment. Our AppBuddy platform is compatible with OpenAI Gym and includes a suite of mobile apps and benchmark tasks that supports a diversity of RL research in the mobile app setting.

==> macros/notations.tex <==
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{xspace}

% General math
\newcommand{\expect}{\mathbb{E}}
%\newcommand{\prob}{\mathbb{P}}
\newcommand{\prob}{\text{Pr}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\tuple}[1]{\langle{#1}\rangle}
\DeclareMathOperator*{\arity}{arity}
\newcommand{\literals}[1]{\mathsf{lit}(#1)}
\newcommand{\Lang}[1]{\mathcal{L}_{#1}}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\defeq}{\triangleq}

% MDPs
\newcommand{\mdp}{\tuple{S,A,r,p,\gamma}}
\newcommand{\strl}{\tuple{S,A,T,\gamma,\mathcal{P},L,\varphi}}
\newcommand{\mtrl}{\tuple{S,A,T,\gamma,\mathcal{P},L,\Phi}}

\newcommand{\qapprox}{\tilde{q}}
\newcommand{\Qapprox}{\widetilde{Q}}

\newcommand{\decoration}{\ding{91}\xspace}


==> old sections/old_design.tex <==
\section{System Design}~\label{sec:design}
% Problem formulation
% V1
%Our objective is to train an RL agent to accomplish tasks in mobile apps it has not seen previously by interacting with (either a physical or an emulated) phone environment. To do this, we design the prerequisite RL building blocks: \textit{state representation, action space, and reward specification.}
% V2
%Our objective is to explore whether an RL agent can learn to accomplish tasks in mobile apps by interacting with (either a physical or an emulated) phone environment. To do this, we design the prerequisite RL building blocks: \textit{state representation, action space, and reward specification.}
% V3
Our objective is to explore whether an RL agent can learn to accomplish tasks in mobile apps by interacting with (either a physical or an emulated) phone environment. Mobile apps are interesting (and challenging) real-world RL benchmarks. Since they are optimized for accessibility, most tasks can be solved after executing a short sequence of actions. However, the branching factor (i.e., action space) is much larger than in a standard RL benchmark, which leads to a very sparse reward signal. Moreover, interacting with Android emulators is slow. These ingredients make mobile apps a challenging benchmark with interesting structure that, hopefully, RL agents will learn to exploit when solving these problems. 

% \subsection{System Overview}
% V1
%The overview of the system is shown in Figure~\ref{fig:overview}. Our design allows an RL agent to interact with multiple environments, where each environment is an Android emulator. At each step, for each emulator, the agent chooses an on-screen UI element and performs an action -- either typing or tapping. A token is chosen as well and is typed into the chosen element if appropriate. After the agent performs the actions, the environments return \textit{states} derived from the emulators' view hierarchies, and \textit{rewards} that are based on the current state of each emulator relative to the task.
% V2
%The overview of the system is shown in Figure~\ref{fig:overview}. The agent (a neural network trained using PPO) interacts with several Android emulators in parallel to collect experiences. At each step, for each emulator, the agent chooses an on-screen UI element and performs an action -- either typing or tapping. After the agent performs the actions, the environments return \textit{states} derived from the available on-screen information and \textit{rewards} that depend on the current task the agent is solving.
% V3
In this section, we present the basic building blocks to use RL in mobile apps: \textit{action space, state representation and reward specification.} The overview of the system is shown in Figure~\ref{fig:overview}. The agent (a neural network trained using PPO) interacts with several Android emulators in parallel to collect experiences. At each step, for each emulator, the agent chooses to tap on (or type into) a particular element on screen. After the agent performs the actions, the environments return \textit{states} derived from the available on-screen information and \textit{rewards} that depend on the current task the agent is solving.

Some tasks might require typing some particular text. For instance, the task ``\textit{add a new Wi-Fi network named Starbucks}" will require the agent to type \textit{Starbucks} at some point. However, it is practically impossible for an RL agent to discover that typing \textit{Starbucks}, letter by letter, will cause it to receive a reward. To handle this issue, we follow the same standard as in the web-based task literature \cite{shi2017world} and provide the agent with a list of tokens to choose from when typing text. With that, we now describe the action space, state representation, and rewards used in our work.

% states in the environments are updated with the newly generated view hierarchy. At the same time, the environments will assign corresponding rewards to the agent based on the new state. %In the following sections, we will discuss the details of representing the state space and action space. Moreover, we will cover the reward specifications.

% In short, we summarize our designs as follows:
% \begin{itemize}
%     \item \textbf{State Representation}: A list of UI elements and their attributes, which are obtained from the view hierarchy of the current screen.    
%     \item \textbf{Action Space}: The agent selects an index corresponding to a UI element and a token that is typed into a chosen element.
%     A list of editable and clickable elements with optional tokens. 
%     \item \textbf{Reward Specification}: The agent is rewarded when it reaches certain intermediate states or accomplishes the task successfully.  
% \end{itemize}

\begin{figure}[tb]
\centering
	\includegraphics[width=0.65\columnwidth]{figs/appbuddy_overview.pdf}
	\caption{The system overview of \our. The environment contains a group of emulators and the states are derived from the view hierarchy of the current screen. In each step, the agent will choose an action, which consists of an element ID and a token, and receive corresponding rewards based on progress made in the task.}
	\label{fig:overview}
% 	\squeezeup
\end{figure}


\subsection{Action Space}
% V1
% We only consider editable/clickable elements.
% Each action that the agent chooses is a tuple that contains 
% {\color{blue}The actions at the agent's avail are tuples comprising a UI element index and a token as shown in Figure~\ref{fig:overview}. The element index ranges from 0 to $n$-$1$, where $n$ is the fixed upper bound for the number of clickable or editable elements used in our state representation.
% %
% % the max number of clickable or editable UI elements on a screen. $n$ is set empirically and is 20 in our paper. 
% % %
% % Note that the number of on-screen elements varies from screen to screen 
% %
% Instead of choosing an action type explicitly, it is determined according to the selected UI element (corresponding to the chosen index).
% %
% % we decide the action type based on the attribute of the selected UI element. 
% %
% If the UI element is editable, the action type will be `type'. Otherwise, the action type will be `tap'. If the element is neither clickable nor editable, no action is performed.

% Finally, the agent chooses a single token from a set of $k$ tokens (in our experiments, $k$ is 4) that are predefined for each task (e.g., in the settings task, one of the tokens is `Starbucks' since the task is to add a Wi-Fi network with Starbucks as the SSID). If an editable element is selected, the chosen token is typed into the element.}

% V2
The main challenge towards successfully applying RL in smartphones is the unreasonably large action space. Technically, a user might tap on any pixel on the screen. But allowing that level of granularity would make learning infeasible. Fortunately, we can reduce the action space to the set of clickable or editable elements on screen by exploiting the information from the \textit{view hierarchy}\footnote{The view hierarchy is similar to the DOM tree for web pages.}. 

In Android applications, each view is associated with a rectangle on the screen. The view is responsible both for displaying the pixels on the screen as well as handling events in that rectangle. All the views on a certain screen are organized in a hierarchical tree structure, which is also called the view hierarchy. We show a simple example of a view hierarchy in Figure~\ref{fig:view_hierarchy}. In this figure, the left part shows a screenshot of the native Android alarm clock app. On the right, we can see part of the view hierarchy at the top and detailed attributes for the selected view called `ImageButton \{Add alarm\}' at the bottom. The selected view is also highlighted in a red rectangle in the screenshot on the left.

\begin{figure}
\centering
	\includegraphics[width=0.65\columnwidth]{figs/view_hierarchy.pdf}
	\caption{An example of the view hierarchy for a given screen. The `+' button with the red border on the left-hand side directly corresponds to the highlighted element (`Add alarm') in the view hierarchy on the right hand side.}
	\label{fig:view_hierarchy}
% 	\squeezeup
\end{figure}

% \commentaj{This is borderline unreadable.  Can we get a higher resolution png?  Or is the issue with the conversion to pdf?}

Since the view hierarchy is always available for any Android application, we use its information to define the action space. From this hierarchy, we automatically extract the list of user interface (UI) elements on the screen that users can tap on or type into. Then, the actions at the agent's avail are tuples comprising a UI element index (w.r.t.\ that list) and a token (as shown in Figure~\ref{fig:overview}). The element index ranges from 0 to $n$-$1$, where $n$ is a fixed upper bound for the maximum number of \textit{clickable} or \textit{editable} elements on any screen. Note that a UI element is \textit{clickable} if it reacts when tapped and a UI element is \textit{editable} if text may be typed into it. When the agent chooses to interact with some UI element, the agent will \textit{type} into that element if the element is \textit{editable} and \textit{tap} on that element if the element is \textit{clickable}. %(all this information is available in the view hierarchy). 

%Since the view hierarchy is always available for any Android application, we use its information to define the action space. The actions at the agent's avail are tuples comprising a UI element index and a token (as shown in Figure~\ref{fig:overview}). The element index ranges from 0 to $n$-$1$, where $n$ is a fixed upper bound for the maximum number of \textit{clickable} or \textit{editable} elements on screen. If the agent chooses to interact with some UI element, the agent will \textit{type} on that element if the element is \textit{editable} and \textit{tap} on it if the element is \textit{clickable} (all this information is available in the view hierarchy). 

In addition to selecting a UI element index, the agent also chooses a single token from a set of $k$ tokens (in our experiments, $k$ is 4) that are predefined for each task. For instance, if the task is ``\textit{add a new Wi-Fi network named Starbucks}," then \textit{Starbucks} will be among the $k$ tokens for that task. Then, the chosen token is typed into the selected UI element if that element is editable. Note that it is also possible to train the agent to select correct tokens from natural language commands (e.g., \cite{jia2019dom}). Finally, while we only consider in this work two types of actions -- tapping and typing, future work will explore action types such as swiping and long tapping.

\subsection{State Representation}
% V1
%In Android applications, each view is associated with a rectangle on the screen. The view is responsible both for displaying the pixels on the screen as well as handling events in that rectangle. All the views on a certain screen are organized in a hierarchical tree structure, which is also called the \textit{view hierarchy}\footnote{The view hierarchy is similar to the DOM tree for web pages.}. We show a simple example of a view hierarchy in Figure~\ref{fig:view_hierarchy}. In this figure, the left part shows a screenshot of an Android phone. On the right is part of the view hierarchy at the top and detailed attributes for the selected view called `TextView:Settings' at the bottom. The selected view is also highlighted in a red rectangle in the screenshot on the left.
%
%A view hierarchy is a well organized structure and provides rich information about the user interface (UI) elements on the screen including their attributes and their relative locations in the tree. We derive the state representation from the view hierarchy extracted from the current screen. We extract from the view hierarchy a list of UI elements, and select a number of salient attributes for each element as shown in Figure~\ref{fig:state_rep}. First, from each UI element in the view hierarchy, we extract the textual description and embed it with a pretrained BERT model~\cite{devlin2018bert,xiao2018bertservice}. Typically, the textual description specifies the purpose of the UI element and is often used to enhance accessibility. Second, we include information about whether an element is \textit{clickable} or \textit{editable} (i.e., the element accepts accept textual input), which helps guide the agent to act on the corresponding elements. Third, we record the relative location of each element, which is the sum of the element's pre-order and post-order tree traversal indices in the view hierarchy. This helps capture the spatial correlations across different UI elements. 

% V2
As explained above, the action space is defined by the list of editable or clickable UI elements in the current screen, which is extracted from the screen's view hierarchy. To represent the state, we use the same list of UI elements. Concretely, the state is represented by a $n\times m$ matrix, where each row is a vector of $m$ features representing a particular UI element from the list and $n$ is an upper bound for the maximum number of clickable or editable elements that we expect to see on any screen. In the matrix, each UI element is represented using $m$ features. These features include the \textit{textual description} of the UI element (which is embedded using a pretrained BERT model~\cite{devlin2018bert}). This description is available in the view hierarchy and specifies the purpose of the UI element (e.g., \textit{`Add alarm'} for the `+' button in Figure~\ref{fig:view_hierarchy}). We also include information about whether the UI element is \textit{clickable} or \textit{editable} and its relative location in the view hierarchy (defined as the element's pre-order tree traversal index). The relative location features help capture the spatial correlations across different UI elements. The process of extracting these features from the view hierarchy is illustrated in Figure~\ref{fig:state_rep}. In our experiments, $m$ is 871, i.e., 768 (BERT) + 3 (clickable/editable) + 100 (location in the view hierarchy).
% summary of features in Figure~\ref{fig:state_rep}).

% V1
% Importantly, we leverage the rich information in the view hierarchy and prune elements that are neither clickable nor editable. Since the number of on-screen elements varies from screen to screen, we choose a fixed upper bound $n$ for the number of editable or clickable elements in the state representation. So, our state representation is a list comprising $n$ elements, where each element is either clickable or editable and contains the three aforementioned components (i.e., BERT-embedded textual description, clickable/editable property, and the element's position in the view hierarchy). 
% % Importantly, we leverage the rich information in the view hierarchy and only include in this list elements that are either editable or clickable
% %
% % Lastly, wf hen training a multi-task agent, besides information related to the UI elements, we also include the natural language-based goal statement, also encoded by BERT, as part of the state representation.
% %
% If a screen has $m < n$ clickable or editable elements, all elements $i > m$ in the state representation are represented by \textcolor{red}{zeroed out vectors.}
% % fewer than $n$ elements, all 

% % The element index varies from 0 to $n$-$1$, where $n$ is the max number of clickable or editable UI elements on a screen. $n$ is set empirically and is 20 in our paper. Note that the number of on-screen elements varies from screen to screen 
% V2
Note that we order the state representation to match the actions in the sense that selecting action $i$ means interacting with the UI element represented by the $i$-th row of the feature matrix. Also, there are cases where the current screen has fewer than $n$ clickable or editable elements. In those cases, we fill the remaining rows of the feature matrix with zeros and, if the agent chooses to interact with nonexistent UI elements, a no-op action is perform (i.e., an action that does not change the environment).

% to the limitations of accessibility mechanisms

% (including spatial correlations of elements and information that is not present in the view hierarchy and is only obtainable from the pixels comprising the screen) 

\begin{figure}
\centering
	\includegraphics[width=0.8\columnwidth]{figs/state_action.pdf}
	\caption{Each clickable or editable element is represented in our state representation by features derived from the view hierarchy of the current screen.}
	\label{fig:state_rep}
% 	\squeezeup
\end{figure}


% - a textual description, 
% 	derived from the current sc
% 	An example of a state representation derived from the view hierarchy of a given screen of an alarm clock app. .... illustration of how feautres for every element are derived from the view hierarchy for the current screen
% 	\commentaj{This does not seem to be an example state representation (which would be an n x m array of items).  What exactly does it depict? The extraction of various features that make up a state?}

\subsection{Reward Specification}
%
% When training a multi-step task without \textcolor{red}{reward shaping}, the agent will only receive the final reward when the task is completed successfully and get zero reward, otherwise. In this case, the reward is very sparse during the training process.

When learning to accomplish tasks in mobile apps, reward is extremely sparse if the agent is only given a positive reward when accomplishing the task and a reward of 0, otherwise.
%
% , the reward is extremely sparse in mobile app tasks. 
%Therefore, here we explore several options for reward shaping to improve the training efficiency. 
%
%In \our, the agent is given a reward based on the view hierarchy following an execution of an action. The environment returns a reward based on the state derived from the view hierarchy.
%
%our setting The RL agent will only receive a reward if it successfully accomplishes the goal, so it is a sparse reward problem
%
To mitigate for reward sparsity, we specify the reward function $R$ such that the agent is given an intermediate reward for reaching certain states in the app that correspond to sub-goals on the way to accomplishing the task.
%
% \begin{equation}\label{eq:reward_spec}
%     R = w_1 * r_{success} + w_2 * r_{intermediate}
% \end{equation}
$R$ is calculated as follows:
\begin{equation}\label{eq:reward_spec}
    R = \sum_{i=0}^{k-1} (w_i \times r_{i}) + w_k \times r_{k} ,
\end{equation}
where $\textbf{w}=\{w_0, w_1,...,w_k\}$ indicates whether the agent has reached a certain state and $\textbf{r}=\{r_0, r_1,...,r_k\}$ represents the rewards. $k$ is the total number of intermediate steps where the agent will receive positive intermediate rewards. The value of $k$ is task-specific. Note that an intermediate reward $r_i$ may only be given once in an episode and $w_i$ is set to 0 after that. %\textcolor{red}{mention reward shaping and that we observed that it did not work well in practice? mention reward hacking?}
%{\color{red}Our reward specification was inspired by reward shaping (e.g., \citeauthor{ng1999policy}, \citeyear{ng1999policy}), which we found to be ineffective and susceptible to reward hacking.} 
%any $r_i$/$w_i$ is only given once per episode. 
%
$r_{k}$ is the reward returned by the environment when the task is complete (based on the view hierarchy extracted from the emulator).\footnote{We also tried using reward shaping to generate intermediate rewards but the results were not as good \cite{ng1999policy}.}

For example, in order to accomplish a task in the settings app in our benchmarks, an agent must add a new Wi-Fi network named `Starbucks'. $w_0 = 1$ when the agent reaches the `Wi-Fi settings' screen and $w_1 = 1$ when the agent reaches the `add new Wi-Fi network' screen. $w_2 = 1$ if the agent has added a new Wi-Fi network called `Starbucks' and it now appears on the screen.
In the next section, we discuss our experiments where we show the impact of excluding intermediate rewards (i.e., where only $w_k = 1$ and, hence, the agent receives a sparse reward for accomplishing the task). 
%
%\textcolor{red}{The various $r_i$, $i < m$, were set empirically, were always smaller than $r_m$, and grew larger as their corresponding states neared the goal state (i.e., when $w_m = 1$).}


% the agent receives when the task i for the agent when the environment determines that the task is complete based on the view hierarchy.
% results comparing between reward specifications that  with only $r_{success}$ as the final reward. 
%and then we have $r_{success}$ which gets bigger as the agent nears the goal and this is task dependent
% only baseline where w1 is 1 w2 is 0

% \textbf{Challenges}
% large branching factor; short optimal plans; sparsity of reward

% \textbf{Reward Specification}
% The agent is given a reward based on the view hierarchy following an execution of an action. 

% our setting The RL agent will only receive a
% reward if it successfully accomplishes the goal, so it is a sparse reward problem

% Instead, we specify the reward such that the agent is given an intermediate reward for reaching certain states in the app that correspond to ***sub goals on the way to achieving the final goal.***

% \textbf{then talk about intermediate rewards}

% % \textbf{Automatic Reward Shaping}


% % \textbf{RM-based Reward Shaping}



==> sections/oldrelated.tex <==
\section{Related Work}
\label{sec:related-work}
%
RL has been applied in the past to web-based tasks that share a number of characteristics with our mobile app setting \cite{shi2017world,liu2018reinforcement,gur2018learning,jia2019dom}. 
%Similar to the mobile app setting
As in our setting, learning to accomplish tasks on the web suffers from sparse reward, and 
%
%as well as the varying number of actions between states. 
%
as in our work, several of these efforts leverage an underlying tree representation of aspects of the state (in our case, the phone's screen, in the case of the web, the current HTML page) in the state representation given to the RL agent. While our work shares some of its motivation with this body of work, our mobile app setting presents a number of unique challenges, including expensive and slow interaction with the environment.

%Like this body of previous work, we also leverage the underlying tree representation of the current screen (in our case, the phone's screen, while in their case it is the current HTML page) in the state representation given to the RL agent. While our work shares some of its motivation with this body of work, we address a mobile setting which presents a unique set of challenges, including expensive and slow interaction with the environment.


% merkle2019cooperative
% a novel setting for RL

% which presents a unique set of challenges, including expensive and slow interaction with the environment, as well as \textcolor{red}{sparse rewards and large action space.}

% \textbf{Table 1 in \cite{liu2018reinforcement} shows some pretty long tasks (some are 12-13 steps long)}

% Moreover, the tasks in our constructed benchmarks, set in a number of mobile apps, are less bounded/

% V1
%There also exists 
Also related, is a body of work that has applied RL to testing mobile apps (e.g., \citeauthor{koroglu2019reinforcement}, \citeyear{koroglu2019reinforcement}; \citeauthor{degott2019learning}, \citeyear{degott2019learning}; \citeauthor{pan2020reinforcement}, \citeyear{pan2020reinforcement}). Similarly to our work, this body of work leverages the underlying representation of apps to facilitate RL training in the mobile setting. Most of these works, however, reward RL agents for crashing or exploring apps (e.g., by identifying valid interactions with on-screen elements or maximizing code coverage by reaching novel states) for testing purposes, rather than reward agents for accomplishing tasks, as we do in this work. 
While \citeauthor{koroglu2019reinforcement} specify concrete test scenarios, their approach uses tabular RL and terminates the learning process when the agent first finds a sequence of actions that satisfies the test scenario. In contrast, here we leverage deep RL to learn policies that consistently accomplish a variety of tasks in mobile apps.

% \citeauthor{romdhana2021deep}, \citeyear{romdhana2021deep} MENTION IN CAMERA READY

% In our setting, it is paramount to 

% , and covering a large number of test scenarios and do not focus on accomplishing useful tasks. 

% (\textbf{\color{red}RT: I think we should provide more details about this body of work because it is the closer to our proposal.})  

% Also, they don't do generalization and I think they don't leverage the view hierarchy in the way we do.}

% and guarantee their correctness

% V1
%Recent work by \citeauthor{li2020mapping} [\citeyear{li2020mapping}] proposed to use supervised learning techniques to learn how to map natural instructions to user interface (UI) elements on the screen of a smartphone. \citeauthor{li2020mapping} adopted crowdsourcing to annotate a dataset coupling natural language instructions (obtained by crawling the web) and corresponding UI elements. By mapping each individual instruction in a sequence of instructions to a UI element, the authors are able to string together individual selections of elements to complete a task. The model assumes that previous steps have been executed correctly when running multi-step tasks. If, for example, the model selects an incorrect UI element at some point along the sequence, then the next prediction will likely fail because the phone is now in an unexpected state ({\color{blue}and the same happens if the app has non-deterministic transitions}). While our work shares its motivation (and some functionality) with \citeauthor{li2020mapping}'s work, we take a different computational approach, namely RL, that does not require extensive annotations of a large dataset. Rather, our RL agent explores mobile apps and receives rewards from the environments that guide it towards accomplishing tasks.
%V2
Recent work by \citeauthor{li2020mapping}~[\citeyear{li2020mapping}] proposed to use supervised learning techniques to learn how to map natural language instructions to user interface (UI) elements on the screen of a smartphone. \citeauthor{li2020mapping} adopted crowdsourcing to annotate a dataset coupling natural language instructions (obtained by crawling the web) and corresponding UI elements. Using that training data, they learn a system that maps instructions into sequences of UI elements to interact with in order to complete a task. The model assumes that previous steps have been executed correctly when running multi-step tasks. If, for example, the model selects an incorrect UI element at some point along the sequence, then the next prediction will likely fail because the phone is now in an unexpected state. While our work shares its motivation (and some functionality) with \citeauthor{li2020mapping}'s work, we take a different computational approach, namely RL, that does not require extensive annotations of a large dataset. Rather, our RL agent explores mobile apps and receives rewards from the environments that guide it towards accomplishing tasks.

% ({\color{blue}and the same happens if the app has non-deterministic transitions})

%(that are either manually \textcolor{red}{or automatically specified})

% and for Google research - they use supervised learning and we use RL

% \noindent The Google Paper
% \begin{quote}
%     contrast to Google - a huge effort went into generating the datasets in their work (including hours upon hours of crowd worker annotation etc.).  In our work, we """" only """ have to define the rewards without annotating this massive amount of data. plus, we can likely automatically specify the rewards from demonstration ( how well this works empirically is to be determined). Beyond that, there's the limitation in their evaluation as discussed where they hardcode the screens given to the model.\\
%      The current state-of-the-art approach proposes a supervised machine learning model to generate the action (i.e., click or type on a certain element) given the current screen and the natural language instruction. However, it needs a large number of training samples to train such a model. Moreover, it always assumes that previous steps have been executed correctly when running multi-step tasks.
% \end{quote}

% \noindent A lots of existing work in MiniWobs - \textbf{Lots of work on web, not much on mobile }

% \begin{itemize}
%     \item RL-based GUI testing 
%         \begin{itemize}
%         \item Reinforcement Learning-Driven Test Generation for Android GUI Applications using Formal Specifications
%         \item Learning User Interface Element Interactions
%         \end{itemize}
% \end{itemize}


